Multi-Objective Deep-Learning-based Biomechanical Deformable Image Registration with MOREA

When choosing a deformable image registration (DIR) approach for images with large deformations and content mismatch, the realism of found transformations often needs to be traded off against the required runtime. DIR approaches using deep learning (DL) techniques have shown remarkable promise in instantly predicting a transformation. However, on difficult registration problems, the realism of these transformations can fall short. DIR approaches using biomechanical, finite element modeling (FEM) techniques can find more realistic transformations, but tend to require much longer runtimes. This work proposes the first hybrid approach to combine them, with the aim of getting the best of both worlds. This hybrid approach, called DL-MOREA, combines a recently introduced multi-objective DL-based DIR approach which leverages the VoxelMorph framework, called DL-MODIR, with MOREA, an evolutionary algorithm-based, multi-objective DIR approach in which a FEM-like biomechanical mesh transformation model is used. In our proposed hybrid approach, the DL results are used to smartly initialize MOREA, with the aim of more efficiently optimizing its mesh transformation model. We empirically compare DL-MOREA against its components, DL-MODIR and MOREA, on CT scan pairs capturing large bladder filling differences of 15 cervical cancer patients. While MOREA requires a median runtime of 45 minutes, DL-MOREA can already find high-quality transformations after 5 minutes. Compared to the DL-MODIR transformations, the transformations found by DL-MOREA exhibit far less folding and improve or preserve the bladder contour distance error.

==> figures/patient-intermediate-excerpt-solution-renders.tex <==
\begin{figure}[b]
    % \vspace{-0.2cm}
    \centering
    \includegraphics[width=0.92\linewidth]{figures/patient-intermediate-excerpt-solution-renders_img.pdf}
    \caption{\footnotesize Renders of the automatically selected registrations of all three approaches, showing transformed contours and inverse DVFs for the patient of the large bladder volume change cluster. For MOREA and DL-MOREA, optimization is terminated after 5 min. Shown are annotated sagittal slices. Arrow color indicates deformation magnitude (see legend). The red rectangle indicates a region of interest in the analysis.}
    \label{fig:patient-intermediate-solution-renders}
    % \vspace{-0.2cm}
\end{figure}

